Proxy-bridged Image Reconstruction Network for Anomaly Detection in Medical Images

Anomaly detection in medical images refers to the identification of abnormal images with only normal images in the training set. Most existing methods solve this problem with a self-reconstruction framework, which tends to learn an identity mapping and reduces the sensitivity to anomalies. To mitigate this problem, in this paper, we propose a novel Proxy-bridged Image Reconstruction Network (ProxyAno) for anomaly detection in medical images. Specifically, we use an intermediate proxy to bridge the input image and the reconstructed image. We study different proxy types, and we find that the superpixel-image (SI) is the best one. We set all pixels' intensities within each superpixel as their average intensity, and denote this image as SI. The proposed ProxyAno consists of two modules, a Proxy Extraction Module and an Image Reconstruction Module. In the Proxy Extraction Module, a memory is introduced to memorize the feature correspondence for normal image to its corresponding SI, while the memorized correspondence does not apply to the abnormal images, which leads to the information loss for abnormal image and facilitates the anomaly detection. In the Image Reconstruction Module, we map an SI to its reconstructed image. Further, we crop a patch from the image and paste it on the normal SI to mimic the anomalies, and enforce the network to reconstruct the normal image even with the pseudo abnormal SI. In this way, our network enlarges the reconstruction error for anomalies. Extensive experiments on brain MR images, retinal OCT images and retinal fundus images verify the effectiveness of our method for both image-level and pixel-level anomaly detection.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec_dis}
\highre{In this section, we conduct more experiments to further verify the effectiveness of our method. The experiments are conducted on the retinal OCT \cite{kermany2018identifying} dataset.}


\vspace{-0.25in}

\highre{
\subsection{Using SI for Anomaly Detection with Proxy Extraction Module}
In our anomaly detection framework, the intermediate SI is essential. To further verify the effectiveness of intermediate SI, we use SI to directly predict the anomaly score. To this end, we design a baseline with only the Proxy Extraction Module. During the training, the input and output of the baseline model are the normal image, and its corresponding SI, respectively. During the test, we compute the prediction error between the SI predicted with trained Proxy Extraction Module, and the SI computed with SLIC \cite{achanta2012slic} algorithm. 
We use the Proxy Extraction Module in two ways, \ie, with and without memory. The results are reported in Table \ref{table_si_PE}.
No matter with or without memory, using SI to directly predict the anomaly score outperforms the Auto-Encoder, verifying the effectiveness of SI.
}

\begin{table}[hhh]
	\centering
%	\small
	\footnotesize
	\caption{\highre{The AUC results of using SI for anomaly detection. Here, only the Proxy Extraction Module is used while the Image Reconstruction Module is not used.}}
	\begin{tabular}{c|c}
		\hline
		Methods &  AUC \\  \hline
		Proxy Extraction Module w/o memory  & 0.811     \\ 
		Proxy Extraction Module w/ memory & 0.837       \\ \hline
		Auto-Encoder \cite{baur2018deep} & 0.783 \\ 
		Our Final Model & 0.933 \\ \hline 
	\end{tabular}
	\label{table_si_PE}
\end{table}

%\highre{
%\subsection{Would SIR-Ano Work for Texture Anomaly?}
%There are about 2 types of anomalies, \ie, structure anomaly and texture anomaly \cite{bergmann2019mvtec}. The anomalies in the medical image are mainly the structure anomaly \cite{zhou2020encoding}. Since SI can preserve the local structure \cite{forsyth2002computer, mori2004recovering}, we propose to leverage SI for medical anomaly detection. 
%The previous experiments verify the effectiveness of our method for structure anomaly. To study the performance of our method for texture anomaly, we apply our method on the texture categories of the MVTec AD dataset \cite{bergmann2019mvtec}.
%The qualitative results are shown in Fig. \ref{fig_texture}. We can observe that the texture anomaly in wood and grid can be roughly detected, while the texture anomaly in carpet and tile cannot be detected. These results show the limitation of our method.
%}

%\begin{figure}[htb]
%	\centering
%	\includegraphics[width=.5\textwidth]{figures/fig_texture}
%	\caption{\highre{Illustration of different types of proxy. Compared with smooth image and smooth patches (short for image with smooth patches), the SI preserves local structure.}}
%	\label{fig_texture}	
%\end{figure}



%\subsection{Information Bottleneck}
%
%\subsection{The connection with AE}
%
%\subsection{The connection with constrained AE}

==> sections/intro_bk.tex <==
\section{Introduction}
Anomaly detection aims to identify abnormalities with only normal data in the training set \cite{chandola2009anomaly}, and recently it has drawn much attention in the community of medical image analysis \cite{schlegl2017unsupervised, zimmerer2019unsupervised, baur2020bayesian, chen2020unsupervised}. 
There are two reasons for this: firstly, it is not easy to acquire medical data, especially for some rare diseases; secondly, it is expensive to annotate the lesion. On the contrary, it is comparatively easier to collect the data from healthy subjects. 
Because of the data constraint, anomaly detection in medical images is more challenging than disease classification that has been well tackled with deep convolutional neural networks (CNNs) \cite{li2019canet, luo2020deep, srinivasan2014fully}.

\todo{R2-C3}
To tackle the anomaly detection with only normal data, \highre{many methods have been proposed. These methods can be roughly categorized into two groups, that is, non-reconstruction paradigm and self-reconstruction paradigm.
Among the non-reconstruction paradigm, Ouardini \etal \cite{ouardini2019towards} proposed an effective transfer-learning based approach for anomaly detection. Golan \etal \cite{golan2018deep} proposed to learn a meaningful representation of the learned training data in a fully discriminative fashion using the self-labeled dataset.
In the self-reconstruction paradigm, a model is trained to reconstruct the normal images \cite{pang2021deep, chalapathy2019deep}. Thus, the reconstruction error of abnormal images is thus larger than the normal ones during the test.
In this work, we focus on the self-reconstruction paradigm anomaly detection on medical images. 
Among the self-reconstruction paradigm, the Auto-Encoder (AE)
} is commonly used for anomaly detection \cite{baur2018deep, zhou2017anomaly}. In the training phase, the AE is learnt with only normal data, and it is expected that the reconstructed image from the decoder will be close to the input for the normal image, and the output is different from the input for the abnormal images in the test phase. 
In addition, generative adversarial network (GAN) \cite{goodfellow2014generative} based approaches have also be introduced to guarantee the fidelity of the reconstruction for normal data \cite{chen2018unsupervised, schlegl2017unsupervised}. Further, other than measuring the anomaly with reconstruction error in the image space, Akcay \etal \cite{akcay2018ganomaly} proposed to append another encoder to extract latent features corresponding to the reconstructed image, and take the difference of latent features corresponding to the input and reconstructed image as the anomaly measurement. 
However, it is worth noting that self-reconstruction is essentially to learn an identity mapping function, and it cannot guarantee the large reconstruction error for abnormal images. Therefore, self-reconstruction based anomaly detection may not be sensitive to anomalies.

\begin{figure}[ttt]
	\centering
	\includegraphics[width=.48\textwidth]{figures/fig_intro}
	\vspace{-0.1in}
	\caption{
	The examples of the normal samples (original image, segmented superpixels, superpixel-image and reconstruction) and abnormal samples in brain MRI and retinal OCT.
	Here the superpixel-image (SI) means the image consists of superpixels colored with the average intensity in each superpixel.
	}
	\vspace{-0.1in}
	\label{fig1}
\end{figure}

To mitigate the identity mapping problem in self-reconstruction based anomaly detection, we propose to use the superpixel-image (SI) as an intermediate proxy for image reconstruction. 

\todo{what is the SI?}
As shown in Fig. \ref{fig1}, we set all pixels' intensities within each superpixel as their average intensity for each superpixel and denote this image as SI. 

\todo{why we need SI?}
On the one hand, SI preserves the local anatomical structure  \cite{forsyth2002computer, mori2004recovering}. One the other hand, the detailed texture information is lost. 
It is expected the mapping between the normal input and its SI follows a pattern, which can be learnt by a neural network.

\todo{how to use SI?}
Based on the SI, we propose a superpixel-image-bridged image reconstruction network (SIR-Ano) for anomaly detection in medical images.
In SIR-Ano, we map the input to an SI by learning a proxy extraction module, and reconstruct the input from SI with an image reconstruction module. By enforcing the network to learn a mapping from normal input to its corresponding SI, it is expected that the network will lead to a large error in SI for an abnormal image, and consequently will lead to a large reconstruction error for an abnormal image, which would favor the anomaly detection. 
In contrast, the reconstruction errors would be small for normal images because the mapping between input and its SI is predictable for them. In this way, our SIR-Ano will avoid the identity mapping issue and preserve the sensitivity to abnormal images.

Specifically, in the proxy extraction module, we introduce a memory to memorize the mapping pattern from the input image to its corresponding SI for normal training data. Given an input, we use its latent feature extracted by the encoder in the proxy extraction module to retrieve the most similar item in the memory, and feed the retrieved feature into the decoder in proxy extraction module to predict the SI. 
Then we feed the SI into the image reconstruction module to reconstruct the input image. 
To further enlarge the reconstruction error for abnormal images, we create pseudo abnormal SI by cutting a patch from a randomly selected normal image and pasting the patch on the normal proxy. Other than the reconstruction from the normal SI, we also enforce the network can well reconstruct the input even with the pseudo abnormal SI. 
In this way, the image reconstruction module would have the ability to repair anomaly, which would result in a large reconstruction error for abnormal images and help the anomaly detection. Experiments on the images of different modalities validate the effectiveness of our approach for both image-level and pixel-level anomaly detection.

The main contributions are summarized as follows:

\begin{enumerate}
	\item To mitigate the identity mapping problem in self-reconstruction based anomaly detection, under the assumption that the mapping from an image and its SI can be predictable for the normal images while the mapping for abnormal images cannot be predicted, we propose the SIR-Ano to connect the input and the reconstructed input with an SI.
	\item In the proxy extraction module, we introduce a memory to memorize the correspondence between the input image and its SI for normal images, while the memorized correspondence does not apply to the abnormal images. 
	\item In the image reconstruction module, a pseudo abnormal SI is built to enforce the network to reconstruct the normal input even with the abnormal SI. This would further enlarge the reconstruction error for abnormal image.
	\item Extensive experiments on three modalities (i.e., brain MRI, retinal OCT and retinal fundus) demonstrate the effectiveness of our approach for anomaly detection. Moreover, to the best of our knowledge, \highre{our work is the first one to verify the effectiveness of pixel-level anomaly detection (\ie, abnormal region segmentation) task on retinal fundus images}.
\end{enumerate}


The rest of this paper is organized as follows:
In Section \ref{sec_related}, we introduce work related to anomaly detection in medical images.
In Section \ref{sec_method}, we detail our proposed SIR-Ano for anomaly detection.
In Section \ref{sec_exp}, extensive experiments on three modalities are conducted to validate the effectiveness of our method.
We conclude our work in Section \ref{sec_clu}.

